Imbalanced Classification via a Tabular Translation GAN

When presented with a binary classification problem where the data exhibits severe class imbalance, most standard predictive methods may fail to accurately model the minority class. We present a model based on Generative Adversarial Networks which uses additional regularization losses to map majority samples to corresponding synthetic minority samples. This translation mechanism encourages the synthesized samples to be close to the class boundary. Furthermore, we explore a selection criterion to retain the most useful of the synthesized samples. Experimental results using several downstream classifiers on a variety of tabular class-imbalanced datasets show that the proposed method improves average precision when compared to alternative re-weighting and oversampling techniques.

==> content/experiments.tex <==
\label{sec:experiments}

% \label{sec:others}
% See Section \ref{sec:headings}.
We evaluate the classification performance of the proposed model under several different regimes of classifier model type, dataset, and imbalance ratio. 

The alternative approaches that we compare to are: Re-weighting (RW) - the baseline approach where the chosen classifier is trained with re-weighting applied on the loss function to maximize performance on a balanced testing criterion, Random Oversampling (ROS) where the minority class is randomly oversampled so as to match the size of the majority class, SMOTE \cite{chawla2002smote}, Borderline SMOTE (B-SMOTE) \cite{han2005borderline}, and SUGAR \cite{lindenbaum2018geometry}.

For each experiment, we record values of the mean average precision (mAP) metric. In the result tables, we also note characteristics of the datasets ($N$ = \# of samples, IR = imbalance ratio). For the tabular translation GAN model, choices for the loss coefficient hyperparameters and selection hyperparameters are chosen via a hyperparameter search using Optuna \cite{akiba2019optuna} on a validation set. Hyperparameter specifications are detailed in \cref{appendix}.
% \begin{itemize}
%     \item Re-weighting (RW) - a baseline approach where the chosen classifier is trained with re-weighting applied on the loss function to maximize performance on a balanced testing criterion.
%     \item Random Oversampling (ROS) - the minority class is randomly oversampled so as to match the size of the majority class
%     \item SMOTE \cite{smote}
%     \item Borderline SMOTE (B-SMOTE) \cite{b-smote} 
%     \item SUGAR \cite{sugar}
% \end{itemize}




In all experiments, pre-processing consisted of normalizing the features and handling categorical features. In the first and second set of experiments, categorical features were one-hot encoded, while in the third set the categorical features were target-encoded using the Category Encoders \cite{mcginnis2018category} package. In addition, in the third set missing feature values were imputed with the mode of the feature, and the Yeo-Johnson transformation \cite{yeo2000new} was applied to features that were determined to follow a power law distribution - specifically,  if over 90\% of the data falls in less than 20\% of the value range of the feature. 


For the first set of experiments, we test the performance of a linear SVM classifier on the KEEL \cite{alcala2011keel} collection of datasets. The scikit-learn \cite{pedregosa2011scikit} implementation is used and loss weights are balanced accordingly to compensate for imbalance. Examining the results in \cref{tab:keel-results}, we find that the proposed model outperforms all others in terms of mAP and median rank, performs the best on the highest number of datasets and is not the worst-performing approach on any dataset.

\begin{table*}[hbt!]
    \fontsize{11pt}{13pt}\selectfont
	\caption{Classification performance on CelebA dataset}
	\vskip 0.15in
	\centering
	\begin{tabular}{lllllllll}
		\toprule
		\multicolumn{3}{c}{Dataset characteristics}  &     \multicolumn{3}{c}{mAP}             \\
		\cmidrule(r){1-3}
		                  % \\
% 		\cmidrule(r){4-6}
		Dataset   & N & IR & RW & ROS & SMOTE & B-SMOTE & SUGAR & TTGAN \\
		\midrule
		CelebA & 203k & 40  & 0.4431 & 0.3918 & 0.3885 & 0.3773 & 0.4062 & \textbf{0.4444} \\
		CelebA (extreme imba.)   & 199k & 200 & 0.1435 & 0.1243 & 0.0944 & 0.0981 & 0.1254 & \textbf{0.1445}   \\
		\bottomrule
	\end{tabular}
	\label{tab:celeba-results}
	\vskip -0.1in
\end{table*}

\begin{table*}[hbt!]
    \fontsize{11pt}{13pt}\selectfont
	\caption{Classification performance on proprietary datasets}
	\vskip 0.15in
	\centering
	\begin{tabular}{lllllllll}
		\toprule
		\multicolumn{3}{c}{Dataset characteristics}  &     \multicolumn{2}{c}{mAP} & \multicolumn{2}{c}{AUC-ROC} & \multicolumn{2}{c}{Precision @ 0.4 Recall}          \\
		                  % \\
		\cmidrule(r){1-3}
		\cmidrule(r){4-5}
		\cmidrule(r){6-7}
		\cmidrule(r){8-9}
		Dataset   & N & IR  & Baseline & TTGAN & Baseline & TTGAN & Baseline & TTGAN\\
		\midrule
		Churn & 6.3M & 23  & 0.255 & \textbf{0.266} & 0.852 & \textbf{0.856} & 0.276 & \textbf{0.282} \\
		Task 1 Return   & 45.3M & 200  & 0.12 & 0.12 & 0.928 &  0.928 & 0.132 & 0.132 \\
		Task 1 Pay & 45.3M & 200  & 0.215 & \textbf{0.219} & 0.946 & 0.946 & 0.239 & 0.239 \\
		Task 2 Return & 60M & 220  & \textbf{0.093} & 0.092 & 0.918 & 0.918 & 0.104 & \textbf{0.105} \\
		Task 2 Pay & 60M & 220  & 0.127 & \textbf{0.132} & 0.946 & \textbf{0.947} & 0.105 & \textbf{0.113} \\
		\bottomrule
	\end{tabular}
	\label{tab:exp3-results}
	\vskip 0.1in
\end{table*}

The second set of experiments involves applying the state-of-the-art Catboost \cite{catboost} boosted trees model on a version of the large CelebA dataset where the features are annotated attributes rather than pixel values, and the target is another attribute \cite{liu2015faceattributes}. We also use an artificially extreme-imbalanced version of this dataset derived by withholding minority samples. Catboost is trained with the F1 loss function, a learning rate of 0.2, for 50 iterations with depth 3 trees. The results are recorded in \cref{tab:celeba-results}.
Here we see a clear advantage of the robustness of the proposed approach when compared to the alternatives: while the other approaches suffer degradation compared to the baseline approach, the tabular translation GAN instead provides a marginal performance improvement over the strong baseline model.


In the third set of experiments, we tested our method on proprietary datasets collected by a large, business-to-consumer organization. The datasets, concerning customer behavior, were collected and preprocessed over the course of several months. The purpose of these datasets is to perform several classification tasks: predicting customer churn (turnover), returning within a specified time interval (Return) and probability to pay within a specified time interval (Pay). Each of these datasets is very large, ranging from 6.3 million samples to 60 million samples, and they each exhibit imbalance ranging from an imbalance ratio of 23 to an extreme imbalance ratio of 220. Improving upon the Catboost-based baseline on these challenging tasks directly affects the ability of the organization to better understand its customers and to take appropriate steps to cater to them. We measure performance on the metrics of AUC-ROC, mAP, and Precision @ 0.4 recall. In the results shown in  \cref{tab:exp3-results}, we see a noticeable improvement on the primary dataset of focus, customer churn. The other datasets exhibit performance that either remains the same or more modestly improves; these datasets are large with varying characteristics and exhibit extreme imbalance. We also note that the mechanism of synthetic sample selection was slightly modified during these experiments: instead of $p_{max}$ representing an upper bound, samples were selected to be as close as possible to $p_{max}$ on either side of it; this improved performance but the interpretation of $p_{max}$ as a parameter that constrains the sample threshold remains unchanged.




Lastly, we also use the UMAP \cite{mcinnes2018umap-software} dimensionality reduction technique to visualize samples from the yeast4 \cite{alcala2011keel} dataset to better understand classification improvement. We compare an identical number of synthetic samples generated by a vanilla GAN and TTGAN respectively. This visualization, shown in \cref{fig:vis}, demonstrates that TTGAN leads the synthesized points to be closer to the class boundary than with a vanilla GAN. A results comparison is given in \cref{tab:vis}.



\begin{figure*}
	\centering
    \input{plots/plot_vanilla_umap_yeast4.tex}
    % \hspace{3pt}
    % \vskip 0.1in
    \hspace{3pt}
    \input{plots/plot_ttgan_umap_yeast4.tex}
    \vskip 0.1in
    \definecolor{majcol}{RGB}{68,1,84}
    \definecolor{mincol}{RGB}{33,145,140}
    \definecolor{gencol}{RGB}{253,231,37}
    % \definecolor{majcol}{RGB}{85, 168, 104}
    % \definecolor{mincol}{RGB}{76, 114, 176}
    % \definecolor{gencol}{RGB}{221, 132, 82}
    \centering
\tikzset{
        leg/.style={
            circle, scale=0.6, line width=0.2mm, draw=black
        },
        }
\begin{tikzpicture}
\begin{axis}[colormap/viridis, ticks=none, width = \legendsize, height = 2cm, xmin=0, xmax=20, ymin=0, ymax=5, draw=white!80!black]
    \node[leg, fill=majcol] at (1,2.5) (blah) {};
    \node[font=\small, right=0.05em of blah] (maj_tag) {Majority};
    \node[leg, fill=mincol, right=0.6em of maj_tag] (blah2)  {};
    \node[font=\small, right=0.05em of blah2] (min_tag) {Minority};
    \node[leg, fill=gencol, right=0.6em of min_tag] (blah3) {};
    \node[font=\small, right=0.05em of blah3] (gen_tag) {Generated Minority};
        % the plots of the functions follow
        % \addplot {x};
        % \addlegendentry{}
        % \addplot {x+4};
        % \addlegendentry{$x+4$}
        % \addplot {2*x};
        % \addlegendentry{}
        % \addplot {2*x+4};
        % \addlegendentry{$2x+4$}
        % \addplot {4*x};
        % \addlegendentry{}
        % \addplot {4*x+4};
        % \addlegendentry{$4x+4$}
\end{axis}
\end{tikzpicture}
\vskip 0.1in
	\caption{A 2-dimensional visualization using UMAP \cite{mcinnes2018umap-software} of samples from the yeast4 dataset \cite{alcala2011keel}. On the left, synthetic samples are generated by a vanilla GAN; on the right, synthetic samples are generated by TTGAN. TTGAN generates samples from more diverse regions, closer to the class boundary.}
	\label{fig:vis}
\end{figure*}


\subsection{Ablation analysis}



To further analyze the performance of the proposed \cref{alg:alg}, we conduct an ablation test by iteratively removing components of the model: comparing TTGAN to TTGAN without the cyclic and identity losses, and comparing that to a "vanilla" GAN model.
We conduct these tests on the page-blocks-1-3\_vs\_4 dataset from \cite{alcala2011keel}. For all experiments besides the baseline, the number of samples generated was 5.5x the number of original minority, as determined by a hyperparameter search on a validation set. The results are shown in \cref{tab:ablation}, and show that removing components of the model degrades performance.



\begin{table}
	\caption{Linear SVM yeast4 comparison}
	\vskip 0.15in
	\centering
	\begin{tabular}{ll}
		\toprule
% 		\multicolumn{2}{c}{Dataset and hyperparameters}            \\
		                  % \\
% 		\cmidrule(r){4-6}
		Model   & mAP \\
		\midrule
		Vanilla GAN   & 0.5352   \\
		TTGAN & \textbf{0.5770} \\
		\bottomrule
	\end{tabular}
	\label{tab:vis}
	\vskip -0.1in
\end{table}


\begin{table}
	\caption{Linear SVM page-blocks ablation analysis}
	\vskip 0.15in
	\centering
	\begin{tabular}{ll}
		\toprule
% 		\multicolumn{2}{c}{Dataset and hyperparameters}            \\
		                  % \\
% 		\cmidrule(r){4-6}
		Model   & mAP \\
		\midrule
		Baseline & 0.7958 \\
		Vanilla GAN   & 0.8069   \\
		TTGAN w/o cyclic+identity losses & 0.8357 \\
		TTGAN & \textbf{0.8972} \\
		\bottomrule
	\end{tabular}
	\label{tab:ablation}
	\vskip -0.1in
\end{table}



We also note that all datasets in all experiments yielded hyperparameters such that the translation loss and cyclic loss were never simultaneously zero, despite that being an option in the hyperparameter search. This suggests improvement over a vanilla GAN trained on the minority class.

 
